Train Faster, Perform Better: Modular Adaptive Training in Over-Parameterized Models

Despite their prevalence in deep-learning communities, over-parameterized models convey high demands of computational costs for proper training. This work studies the fine-grained, modular-level learning dynamics of over-parameterized models to attain a more efficient and fruitful training strategy. Empirical evidence reveals that when scaling down into network modules, such as heads in self-attention models, we can observe varying learning patterns implicitly associated with each module's trainability. To describe such modular-level learning capabilities, we introduce a novel concept dubbed modular neural tangent kernel (mNTK), and we demonstrate that the quality of a module's learning is tightly associated with its mNTK's principal eigenvalue $\lambda_{\max}$. A large $\lambda_{\max}$ indicates that the module learns features with better convergence, while those miniature ones may impact generalization negatively. Inspired by the discovery, we propose a novel training strategy termed Modular Adaptive Training (MAT) to update those modules with their $\lambda_{\max}$ exceeding a dynamic threshold selectively, concentrating the model on learning common features and ignoring those inconsistent ones. Unlike most existing training schemes with a complete BP cycle across all network modules, MAT can significantly save computations by its partially-updating strategy and can further improve performance. Experiments show that MAT nearly halves the computational cost of model training and outperforms the accuracy of baselines.

==> old_version/1_intro-0516.tex <==
\section{Introduction}

% Over-parameterization exhibits superior performance across different types of deep learning applications in recent works. 
The proliferation of large pre-trained models~\citep{devlin2018bert, brown2020language, dosovitskiy2020image} demonstrates the advantages and practical usage of over-parameterized models. Since the parameters are far larger than the training data, these models can adequately fit the training set~\citep{dugradient}. 
Indeed, recent theoretical studies show that over-parameterization plays an essential role in model optimization and generalization~\citep{liu2022loss}.  
% Furthermore, the mathematical properties governed by the Polyak-{\L}ojasiewicz condition~\citep{polyak1963gradient,liu2022loss} reveal the potential of the optimization of over-parameterized models, which can provably converge to a global minimum by gradient descent-based methods ***Is this a general property or does it require gross over-parameterization. It was my understanding that the transition from a jagged to smooth loss landscape was gradual, with local minima still existing in over-parameterized models but decreasing with more severe over-parameterization.***
% 
However, over-parameterized models are expensive to train.
% Expanding model scale places ever-increasing demands on computation and memory. 
For example, training large language models such as GPT-3~\citep{brown2020language, zaheer2020big} takes weeks to months on a large number of GPUs. 
% This raises a question: {\it Has the computational resource been used efficiently and appropriately during model training?} 
\textcolor{blue}{
{\it The work seeks to optimize over-parameterized models while reducing computation costs.}
}


% Many works also suggest training these models needs extra care~\citep{chen2021empirical, chen2022vision}. 
% 
% In addition, many works report that training these models needs extra care~\citep{chen2021empirical, chen2022vision}.  ***``Extra care'' is very vague. What do you really mean?***
% This raises a question: {\it Has the computational resource been used efficiently and appropriately during model training?} ***This question didn't work very well. Is it better to state an optimization problem or ask this question? If you ask a question, you should make it more precise.***


% Modern practical over-parameterized deep models often have a layer-wise structure consisting of various modules, such as multi-head self-attention~(MHSA) in Transformer~\citep{vaswani2017attention}, experts in mixture-of-experts~(MoE)~\citep{shazeeroutrageously} architecture, and filters in convolutional neural networks~(CNN). In this work, we take a deep dive into the training process of over-parameterized models and investigate the allocation of computational resources at the module level during model training. 
In this work, we take a deep dive into the training process of over-parameterized models by focusing on their modular behavior and seek for an effective strategy for allocating computational resources at the module level during model training. 
Modern practical over-parameterized models have a layer-wise structure consisting of various modules, such as multi-head self-attention~(MHSA) in Transformer~\citep{vaswani2017attention}, experts in mixture-of-experts~(MoE)~\citep{shazeeroutrageously} architecture, and filters in convolutional neural networks~(CNN). 
To better understand the training dynamics at the module level, we propose modular Neural Tangent Kernel~(mNTK), derived from integral NTK~\citep{jacot2018neural, fort2020deep}. 
Modular NTK calculates the gradient correlation among the training data in a particular module, whose eigenspectrum describes the learning dynamics of module parameters. The eigenvalues indicate the degree of consistency in the updates of parameters, with the principal eigenvalue $\lambda_{\max}$ reflecting the update from the most common features of the training samples. ***The previous two sentences were vague. They don't say enough for reviewers who aren't already familiar with the NTK to understand. I think this explantion is also important to paper.***
% The principal eigenvalue $\lambda_{\max}$ indicates the consistency of the parameter updates, corresponding to the most common features of training samples.

% This work opens the hood and takes a deeper dive into the internal training process of fine-grained component level of over-parameterized models.
% Although theoretically the excessive parameters of overall model has the advantage of fitting complex manifold, the components are not necessarily competent learners of local features.
%which is an important tool to analyse training dynamics of the model. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figure/intro.png}
    \caption{***The meaning of shades of gray in (a) is unclear. Additional explanation in the caption might help. (b) is hard to read because the text is too small.*** Characteristics of training BERT on WikiText-2. Figure~(a) demonstrates the joint variation of effective rank and $\lambda_{\max}$ across the attention heads.
    % The head in red maintains low eigenvalue learns few effective information, while the blue one with respectively lower eigenvalue may starts overfitting.
    Head$^l_i$ refers to the $i^\text{th}$ attention head in the $l^\text{th}$ layer.
    Figure~(b-left) illustrates the idea of MAT, which governs the heads training by a dynamic threshold. Using MAT speeds up convergence and achieves lower validation loss (b-right). }
    \label{fig:intro}
\end{figure}

% We demonstrate that the components across the model are highly asynchronized and heterogeneous, which results in the training issues and inappropriate use of computational resources.

% Figure~\ref{fig:intro} characterizes the spatial-temporal training dynamics of the standarded BERT~\citep{devlin2018bert}. The standard BERT has 12 layers, with 12 heads in each layer, and we regard each attention head as a module in this case. Effective rank~\citep{roy2007effective, garrido2022rankme} is a widely used metric to evaluate the amount of effective information ***I presume ``information'' is the formal term. How does ``effective'' modify it? The meaning of ``effective'' is unclear without reference to the cited papers.*** in a matrix, such as attention matrix. As shown in Figure~\ref{fig:intro}, for an attention head, as the largest eigenvalue of its mNTK decreases, its effective rank rises accordingly, i.e., the head continually learns the useful common features. As we can see, this learning process is asynchronizedly distributed in different attention heads, where such a distribution reveals following two properties of model training from the perspective of modules: 
% %To study the characteristics of component-level model training using spatio-temporal distribution of the empirical NTK, 

% \textbf{(1)~Spatially different.}
% % It has been discussed that network will become untrainable if the condition number of the NTK diverges~\citep{xiao2020disentangling}.
% At a specific moment, different modules are active with larger $\lambda_{\max}$. The network is biased to learn the top eigenfunctions of the NTK over the entire input space~\citep{bowman2022spectral}, while the parameters with relatively low eigenvalues updates weakly. In other words, modules with larger $\lambda_{\max}$ show larger consistency over data samples on feature learning, which are apt to converge with better trainability. ***The previous sentence is vague. Do you mean that it converges more rapidly (does that really much matter?) or that it improves accuracy more rapidly?***In the Figure~\ref{fig:intro}, the attention head in red marker learns few information with relatively small effective rank, as its mNTK $\lambda_{\max}$ always oscillates at a low level. This means that some modules learning diverse features may be hard to converge and ineffectively occupy computation cost.

% % Behind these works, we reveal that some ill-conditioned local components in the over-parameterized model may cause poor convergence of the whole model. As shown in fig~\ref{fig:intro}(a), if we dynamically freeze certain poorly-behaved component, the model converges faster with better generalization.

% \textbf{(2)~Temporally dynamic.}
% Every module has its own variation of $\lambda_{\max}$. Modules learn new features or converge at different moments. In the later stage of training, converged modules are prone to continually learn those features specific to the training set corresponding to small eigenvalues, which are difficult to generalize to the test set~\citep{oymak2019generalization}. This causes overfitting, thus impedes the generalization.
% % Generalization means the ability that a neural network predicts the unseen data. Over-fitting is the key reason that impedes generalization when fitting a complex function to a finite dataset.
% For example, the $\lambda_{\max}$ of attention head in blue marker of Figure~\ref{fig:intro} is so small that it's learning features specific to the training set or even noise information. 

% In the over-parameterized model, we find that the temporal variation pattern of NTK reflects the time nodes of local overfitting.Empirical study~\ref{fig:intro}(c) shows that the moment when the model starts over-fit is when the largest eigenvalue of normalized NTK reaches its minumum. Based on this observation, we are inspired that features consistent in the training samples are most important for generalization, which motivates us to adapt the training process by denoising features.

To demonstrate the close relationship between the training dynamic and mNTK, we use the standard BERT~\citep{devlin2018bert} as an example. The standard BERT has 12 layers, with 12 heads in each layer, and we regard each attention head as a module in this case. In addition, we adopt the effective rank~\citep{roy2007effective} as a measure of effective dimensionality of a feature matrix, such as attention matrix; The measure is calculated every training epoch. Figure~\ref{fig:intro} (a) shows the spatial-temporal training dynamics of BERT~\citep{devlin2018bert} in terms of effective rank and $\lambda_{\max}$. Firstly, we notice a clear difference among the effective rank of different heads at different layers. In early stage of training (epoch 5), only heads at lower layers contain some information, which are likely learning the shallow features. In later stage of training (epoch 100),  heads at higher layers contain more information than those at lower layers, and the difference between heads at the same layer becomes more pronounced. Such difference in heads offers the potential for allocating unequal training resources to different modules. Secondly, $\lambda_{\max}$ serves as a good indicator of trainabilty, which means how effectively network parameters can be optimized by gradient descent. As discussed in~\cite{bowman2022spectral}, the network is biased to learn the top eigenfunctions of the NTK over the entire input space, while the parameters with relatively low eigenvalues barely updates. In Figure~\ref{fig:intro} (a), attention heads in blue and green markers have large $\lambda_{\max}$, meaning that they have large consistency over data samples on feature learning and thus apt to converge with better trainability. 
These heads are also more useful ***The meaning of ``more useful'' isn't defined. What does it mean w.r.t. accuracy?*** as reflected through effective rank. 
These heads contain more effective information as reflected through effective rank. 
In contrast, $\lambda_{\max}$ of the red attention head oscillates at a low level, likely as a result of learning diverse features that may be hard to converge
***You are basically repeating what you observed and pretending its an explanation. It doesn't offer insight into the cause.***
, and learns little effective features. 
***This doesn't make sense to me under an information theoretic definition of ``information''. What definition of ``information'' are you using? It's not clear.***
Thirdly, $\lambda_{\max}$ could also indicate generalizability, which means how well the network predicts the unseen data. Every module has its own temporal variation of $\lambda_{\max}$, learning new features and converging at different times. For example, the $\lambda_{\max}$ of attention head in blue marker of Figure~\ref{fig:intro} (a) is so small at the late stage that it may start to learn features specific to the training set or even noise information. 

% Each module has its own training process, and they should not be allocated equal training resources at any time as widely practiced. That's the reason why the existing training scheme fails to train over-parameterized models efficiently.
% which means how well a model optimizes within the certain computation and memory usage.

Our empirical analysis shows that variation of $\lambda_{\max}$ signals the modular training process. Furthermore, we theoretically analyze that the modules with larger $\lambda_{\max}$ are learning features that are more rapidly learned and more effective at generalization. Motivated by these analyses, we propose a simple yet effective training method termed Modular Adaptive Training~(MAT), aiming at dynamically training partial modules to improve training efficiency. As shown in Figure~\ref{fig:intro} (b), we design a dynamic threshold (the dash-dotted line), according to temporal variation of $\lambda_{\max}$ of inter- and intra-module mNTK. MAT only back-propagates the parameters of those modules whose $\lambda_{\max}$ are larger than the threshold. According to the experimental results, MAT saves half of the FLOPs and the model performs better on the test data. 
***Why? Why did omitting updates that would have improved training loss improve test loss? Insight about the cause would be good. Just saying ``overtraining'' isn't a thorough analysis of the cause.***
% , i.e., make the model better optimized within the certain computation. 
% MAT selects modules with larger $\lambda_{\max}$ and only back-propagates these subsets of modules, by which one can obtain large speed-up and alleviate overfitting.
% keep higher spectrum of overall NTK by denoising the smaller eigenvalues.
% In the other word, we concentrate the model on learning the common featrues, which can be analysed to improve convergence and alleviate overfitting.

Our contributions follow. ***Given the focus on accuracy in the field, it might be interesting to look at improvement in test accuracy given the same training time and computational resources. This might be more impressive than halving resource use for some readers.***
\begin{itemize}
    \item We demonstrate and analyze the relationship between fine-grained training dynamics and modular Neural Tangent Kernel~(mNTK), both empirically and theoretically.
    \item We propose a runtime training policy termed Modular Adaptive Training~(MAT), which applies a dynamic threshold to selectively back-propagate part of the network modules for efficient training.
    \item Our method can be applied to various structured over-parameterized models. Experimental results show that the method reduces training computation and improves test performance.
\end{itemize}

***More detail on your findings early in the paper would improve the paper.***

% An adaptive training regime based on these metrics governs which components to update parameters during the whole training process. Experimental results demonstrate that our method helps the over-parameterized model converge faster with less computation usage, meanwhile alleviating the over-fit phenomenon.


==> old_version/1_intro-0517.tex <==
\section{Introduction}

% Over-parameterization exhibits superior performance across different types of deep learning applications in recent works. 
The proliferation of large pre-trained models~\citep{devlin2018bert, brown2020language, dosovitskiy2020image} demonstrates the advantages and practical usage of over-parameterized models. Since the parameters are far larger than the training data, these models can adequately fit the training set~\citep{dugradient}. 
Indeed, recent theoretical studies show that over-parameterization plays an essential role in model optimization and generalization~\citep{liu2022loss}.  
% Furthermore, the mathematical properties governed by the Polyak-{\L}ojasiewicz condition~\citep{polyak1963gradient,liu2022loss} reveal the potential of the optimization of over-parameterized models, which can provably converge to a global minimum by gradient descent-based methods ***Is this a general property or does it require gross over-parameterization. It was my understanding that the transition from a jagged to smooth loss landscape was gradual, with local minima still existing in over-parameterized models but decreasing with more severe over-parameterization.***
% 
However, over-parameterized models are expensive to train.
% Expanding model scale places ever-increasing demands on computation and memory. 
For example, training large language models such as GPT-3~\citep{brown2020language, zaheer2020big} may take weeks to months on a large number of GPUs. 
This raises a question: {\it Has the computational resource been used efficiently for loss minimization during model training?} 
% \textcolor{blue}{
% {\it The work seeks to optimize over-parameterized models while reducing computation costs.}}


In this work, we take a deep dive into the training process of over-parameterized models by focusing on their modular behavior and seek for an effective strategy for allocating computational resources at the module level during model training. Modern practical over-parameterized models have layer-wise structures consisting of various modules, such as multi-head self-attention~(MHSA) in Transformer~\citep{vaswani2017attention}, experts in mixture-of-experts~(MoE)~\citep{shazeeroutrageously} architecture, and filters in convolutional neural networks~(CNN). To better understand the training dynamics at the module level, we propose modular Neural Tangent Kernel~(mNTK), derived from the vanilla NTK~\citep{jacot2018neural, fort2020deep}. 
Modular NTK calculates the first-order approximation of module's evolution during gradient descent training, which captures the gradient correlation among the training data in a particular module. 
Its eigenspectrum describes the learning dynamics of module parameters, with the principal eigenvalue $\lambda_{\max}$ indicating the degree of consistency in the gradient direction for learning the most common features of the training samples.
% Modular NTK calculates the first-order approximation of module's evolution during gradient descent training, which captures the gradient correlation among the training data in a particular module. 
% Therefore, the eigenspectrum of mNTK describes the learning dynamics of module parameters. 
% The eigenvalues of mNTK indicate the degree of consistency in the updates of parameters, with the principal eigenvalue $\lambda_{\max}$ reflecting the update from the most common features of the training samples. 
% ***The previous two sentences were vague. They don't say enough for reviewers who aren't already familiar with the NTK to understand. I think this explantion is also important to paper.***
% The principal eigenvalue $\lambda_{\max}$ indicates the consistency of the parameter updates, corresponding to the most common features of training samples.

% This work opens the hood and takes a deeper dive into the internal training process of fine-grained component level of over-parameterized models.
% Although theoretically the excessive parameters of overall model has the advantage of fitting complex manifold, the components are not necessarily competent learners of local features.
%which is an important tool to analyse training dynamics of the model. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figure/intro.png}
    \vspace{-2em}
    \caption{
    % ***The meaning of shades of gray in (a) is unclear. Additional explanation in the caption might help. *** 
    Characteristics of training BERT on WikiText-2. Figure~(a) demonstrates the joint variation of effective rank and $\lambda_{\max}$ across the attention heads.
    % The head in red maintains low eigenvalue learns few effective information, while the blue one with respectively lower eigenvalue may starts overfitting.
    Head$^l_i$ refers to the $i^\text{th}$ attention head in the $l^\text{th}$ layer.
    Figure~(b-left) illustrates the idea of MAT, which governs the heads training by a dynamic threshold. Using MAT speeds up convergence and achieves lower validation loss (b-right). }
    \label{fig:intro}
\end{figure}

% We demonstrate that the components across the model are highly asynchronized and heterogeneous, which results in the training issues and inappropriate use of computational resources.

% Figure~\ref{fig:intro} characterizes the spatial-temporal training dynamics of the standarded BERT~\citep{devlin2018bert}. The standard BERT has 12 layers, with 12 heads in each layer, and we regard each attention head as a module in this case. Effective rank~\citep{roy2007effective, garrido2022rankme} is a widely used metric to evaluate the amount of effective information ***I presume ``information'' is the formal term. How does ``effective'' modify it? The meaning of ``effective'' is unclear without reference to the cited papers.*** in a matrix, such as attention matrix. As shown in Figure~\ref{fig:intro}, for an attention head, as the largest eigenvalue of its mNTK decreases, its effective rank rises accordingly, i.e., the head continually learns the useful common features. As we can see, this learning process is asynchronizedly distributed in different attention heads, where such a distribution reveals following two properties of model training from the perspective of modules: 
% %To study the characteristics of component-level model training using spatio-temporal distribution of the empirical NTK, 

% \textbf{(1)~Spatially different.}
% % It has been discussed that network will become untrainable if the condition number of the NTK diverges~\citep{xiao2020disentangling}.
% At a specific moment, different modules are active with larger $\lambda_{\max}$. The network is biased to learn the top eigenfunctions of the NTK over the entire input space~\citep{bowman2022spectral}, while the parameters with relatively low eigenvalues updates weakly. In other words, modules with larger $\lambda_{\max}$ show larger consistency over data samples on feature learning, which are apt to converge with better trainability. ***The previous sentence is vague. Do you mean that it converges more rapidly (does that really much matter?) or that it improves accuracy more rapidly?***In the Figure~\ref{fig:intro}, the attention head in red marker learns few information with relatively small effective rank, as its mNTK $\lambda_{\max}$ always oscillates at a low level. This means that some modules learning diverse features may be hard to converge and ineffectively occupy computation cost.

% % Behind these works, we reveal that some ill-conditioned local components in the over-parameterized model may cause poor convergence of the whole model. As shown in fig~\ref{fig:intro}(a), if we dynamically freeze certain poorly-behaved component, the model converges faster with better generalization.

% \textbf{(2)~Temporally dynamic.}
% Every module has its own variation of $\lambda_{\max}$. Modules learn new features or converge at different moments. In the later stage of training, converged modules are prone to continually learn those features specific to the training set corresponding to small eigenvalues, which are difficult to generalize to the test set~\citep{oymak2019generalization}. This causes overfitting, thus impedes the generalization.
% % Generalization means the ability that a neural network predicts the unseen data. Over-fitting is the key reason that impedes generalization when fitting a complex function to a finite dataset.
% For example, the $\lambda_{\max}$ of attention head in blue marker of Figure~\ref{fig:intro} is so small that it's learning features specific to the training set or even noise information. 

% In the over-parameterized model, we find that the temporal variation pattern of NTK reflects the time nodes of local overfitting.Empirical study~\ref{fig:intro}(c) shows that the moment when the model starts over-fit is when the largest eigenvalue of normalized NTK reaches its minumum. Based on this observation, we are inspired that features consistent in the training samples are most important for generalization, which motivates us to adapt the training process by denoising features.

To demonstrate the close relationship between the training dynamic and mNTK, we use the standard BERT~\citep{devlin2018bert} as an example. The standard BERT has 12 layers, with 12 heads in each layer, and we regard each attention head as a module in this case. 
In addition, we adopt the effective rank~\citep{roy2007effective} as a measure of effective dimensionality of a feature matrix, such as attention matrix; the measure is calculated every training epoch. Figure~\ref{fig:intro}(a) presents the trend of training dynamics of BERT in terms of effective rank and $\lambda_{\max}$. 
Firstly, $\lambda_{\max}$ serves as a good indicator of trainabilty, which means how effectively network parameters can be optimized by gradient descent. As discussed in~\cite{bowman2022spectral}, the network is biased to learn the top eigenfunctions of the NTK over the entire input space, while the parameters with relatively low eigenvalues barely updates. In Figure~\ref{fig:intro}(a), attention heads in blue and green markers have large $\lambda_{\max}$, meaning that they have large consistency over data samples on feature learning and thus apt to converge with better trainability. 
Indeed, These heads contain more effective information as reflected through effective rank. In contrast, $\lambda_{\max}$ of the red attention head oscillates at a low level, likely as a result of learning diverse features that may be hard to converge, and learns little effective features.
% we notice a clear difference among the effective rank of different heads at different layers. In early stage of training (epoch 5), only heads at lower layers contain some information, which are likely learning the shallow features. In later stage of training (epoch 100),  heads at higher layers contain more information than those at lower layers, and the difference between heads at the same layer becomes more pronounced. Such difference in heads offers the potential for allocating unequal training resources to different modules. 
Furthermore, $\lambda_{\max}$ could also indicate generalizability, which means how well the network predicts the unseen data. Every module has its own temporal variation of $\lambda_{\max}$, learning new features and converging at different times. For example, the $\lambda_{\max}$ of the attention head in blue marker of Figure~\ref{fig:intro}(a) is so small at the late stage that it may start to learn superfluous features that are too specific or even noise. 

% Each module has its own training process, and they should not be allocated equal training resources at any time as widely practiced. That's the reason why the existing training scheme fails to train over-parameterized models efficiently.
% which means how well a model optimizes within the certain computation and memory usage.

Our empirical analysis shows that variation of $\lambda_{\max}$ signals the modular training process. Furthermore, we theoretically analyze that the modules with large $\lambda_{\max}$ are learning features that are more rapidly learned while those without large $\lambda_{\max}$ have negative influences on generalization in existing training scheme. Motivated by these analyses, we propose a simple yet effective training method termed Modular Adaptive Training~(MAT), aiming at dynamically training partial modules to improve training efficiency. As shown in Figure~\ref{fig:intro}(b), we design a dynamic threshold (the dash-dotted line), according to modular difference and temporal variation of mNTK $\lambda_{\max}$. MAT only back-propagates the parameters of those modules whose $\lambda_{\max}$ is larger than the threshold. This forces the network to concentrate on learning the common features and ignore the inconsistent ones, and also prevent it from fitting superfluous features or noises.
% According to the experimental results, MAT saves half of the FLOPs and the model performs better on the test data. 
% ***Why? Why did omitting updates that would have improved training loss improve test loss? Insight about the cause would be good. Just saying ``overtraining'' isn't a thorough analysis of the cause.***
% , i.e., make the model better optimized within the certain computation. 
% MAT selects modules with larger $\lambda_{\max}$ and only back-propagates these subsets of modules, by which one can obtain large speed-up and alleviate overfitting.
% keep higher spectrum of overall NTK by denoising the smaller eigenvalues.
% In the other word, we concentrate the model on learning the common featrues, which can be analysed to improve convergence and alleviate overfitting.

Our contributions follow. 
% ***Given the focus on accuracy in the field, it might be interesting to look at improvement in test accuracy given the same training time and computational resources. This might be more impressive than halving resource use for some readers.***
\begin{itemize}
    \item We demonstrate and analyze the relationship between fine-grained training dynamics and modular Neural Tangent Kernel~(mNTK), both empirically and theoretically.
    \item We propose a runtime training policy termed Modular Adaptive Training~(MAT), which applies a dynamic threshold to selectively back-propagate part of the network modules for efficient training.
    \item Our method can be applied to various structured over-parameterized models. Experimental results show that the method reduces training computation and improves test performance.
\end{itemize}

% ***More detail on your findings early in the paper would improve the paper.***

% An adaptive training regime based on these metrics governs which components to update parameters during the whole training process. Experimental results demonstrate that our method helps the over-parameterized model converge faster with less computation usage, meanwhile alleviating the over-fit phenomenon.


==> old_version/2_analysis-0517.tex <==
\section{Analysis of Modular Neural Tangent Kernel in Over-Parameterized Models}
In this section, we first introduce the definition of Neural Tangent Kernel (NTK) and modular Neural Tangent Kernel (mNTK). 
Next, we present empirical analysis revealing the eigenspectrum characteristics of the mNTK, including the imbalanced distribution of mNTK eigenvalues and the modular and temporal diversity of mNTK eigenvalues during training.
Finally, we provide theoretical analysis to show that trainability and generalization ability of over-parameterized structured models are closely related to the largest mNTK eigenvalues. 

% Let $\mathcal{X}$ denote the set of all the training data, $\mathcal{Y}$ the target labels generated i.i.d. according to a distribution $\mathcal{D}$. Let $\mathcal{Z}=f(\mathcal{X};\boldsymbol{\theta})$ denote the output of the neural network, $\mathcal{L}$ the loss function. $m$ and $n$ denotes the number of network parameters and training samples and $k$ denotes the output space dimension.
% We define the residual $\boldsymbol{r}_t=f(\mathcal{X} ; \boldsymbol{\theta}_t) - \mathcal{Y}$.
% There has $m\gg n$ in an over-parameterized model~\citep{liu2020toward}.

\subsection{Preliminary}
% Let $\mathcal{X}$ and $\mathcal{Y}$ denote the set of $n$ i.i.d. training instance and label pairs, randomly sampled according to an unknown distribution $\mathcal{D}$. Let $\mathcal{Z}=f(\mathcal{X};\boldsymbol{\theta})$ denote the output of the neural network, $m$ denotes the number of network parameters, and $k$ denotes the output space dimension. In an over-parameterized model~\citep{liu2020toward}, $m\gg n$. Let $\mathcal{L}$ denote the loss function.

Let $\mathcal{X}$ and $\mathcal{Y}$ denote the set of $n$ training instance and label pairs, respectively, which are i.i.d. drawn from an unknown distribution $\mathcal{D}$. 
We study the network function $f$ parameterized by $\boldsymbol{\theta}$ aiming to map the input vector $\mathcal{X}$ to output vector $\mathcal{Z}$, termed as $\mathcal{Z}=f(\mathcal{X};\boldsymbol{\theta})$ where $\boldsymbol{\theta} \in \mathbb{R}^m$ and $\mathcal{Z} \in\mathbb{R}^k$. 
% In an over-parameterized model~\citep{liu2020toward}, $m\gg n$. Let $\mathcal{L}$ denote the loss function.

\begin{definition}
(Neural Tangent Kernel~(NTK)~\citep{jacot2018neural}). We define NTK as $\boldsymbol{\Theta}(\mathcal{X},\mathcal{X})=J_\theta(\mathcal{X})J_\theta(\mathcal{X})^\top$, where $J_{\boldsymbol{\theta}}=\nabla_{\boldsymbol{\theta}} f(\mathcal{X};{\boldsymbol{\theta}}) \in \mathbb{R}^{nk\times m}$ denotes the Jacobian of the function $f$ at the points $\mathcal{X}$ with respect to the flattened vector of all parameters ${\boldsymbol{\theta}} \in \mathbb{R}^{m}$.
\end{definition} 


% Note that $\boldsymbol{\Theta} \in \mathbb{R}^{nk \times nk}$ is a semi-positive definite real symmetric matrix, thus it has $nk$ non-negative eigenvalues $\lambda_{\max}=\lambda_1 \ge\lambda_2 \ge...\ge\lambda_{nk}\ge 0$ by eigendecomposition $\boldsymbol{\Theta}=\mathbf{U} \mathbf{\Lambda} \mathbf{U}^\top=\sum_{i=1}^{nk} \lambda_i \mathbf{u}_i \mathbf{u}_i^\top$. For clarity, NTK is referred to as integral NTK hereafter. For fine-grained analysis of structured deep networks, we introduce modular NTK.
% NTK is widely used to analyze the training dynamics of over-parameterized network. 
It is clear that $\boldsymbol{\Theta} \in \mathbb{R}^{nk \times nk}$ is a positive semi-definite real symmetric matrix. 
Therefore, by eigen-decomposition of NTK $\boldsymbol{\Theta}=\mathbf{U} \mathbf{\Lambda} \mathbf{U}^\top=\sum_{i=1}^{nk} \lambda_i \mathbf{u}_i \mathbf{u}_i^\top$, the eigenspectrum of NTK contains $nk$ non-negative eigenvalues $\boldsymbol{\lambda}(\boldsymbol{\Theta}) = \{\lambda_1,\lambda_2, ..., \lambda_{nk}\}$ with the decreasing order $\lambda_1 \ge \lambda_2 \ge...\ge\lambda_{nk}\ge 0$. 
For clarity, NTK is referred to as integral NTK hereafter. 
Next, we introduce modular NTK for fine-grained analysis of structured deep networks as below.
% \begin{definition}
% (Modular Neural Tangent Kernel~(mNTK)).
% Suppose model $f$ contains $L$ disjoint modules, $\boldsymbol{\theta}^1, \boldsymbol{\theta}^2, ..., \boldsymbol{\theta}^L$. Each of the modules has its own modular NTK $\boldsymbol{\Theta}^1, \boldsymbol{\Theta}^2,..., \boldsymbol{\Theta}^L$, defined by $\boldsymbol{\Theta}^l(\mathcal{X},\mathcal{X})=J_{\boldsymbol{\theta}^l}(\mathcal{X})J_{\boldsymbol{\theta}^l}(\mathcal{X})^\top$.
% \end{definition}
\begin{definition}
(Modular Neural Tangent Kernel~(mNTK)).
Suppose model $f$ contains $L$ disjoint modules $\boldsymbol{\theta} = \{\boldsymbol{\theta}^1, \boldsymbol{\theta}^2, \ldots, \boldsymbol{\theta}^L\}$ where $\boldsymbol{\theta}^l$ denote the parameters of $l^\text{th}$ module. 
We define mNTK as a matrix by $\boldsymbol{\Theta}^l(\mathcal{X},\mathcal{X})=J_{\boldsymbol{\theta}^l}(\mathcal{X})J_{\boldsymbol{\theta}^l}(\mathcal{X})^\top$, where $J_{\boldsymbol{\theta}^l}
=\nabla_{\boldsymbol{\theta}^l} f(\mathcal{X};{\boldsymbol{\theta}^l})$ denotes the Jacobian of the function $f$ at the points $\mathcal{X}$ with respect to the $l^\text{th}$ module's parameters ${\boldsymbol{\theta}^l}$.
\end{definition}
% Note that the division of modules can be flexible. Deep networks can be simply divided by each layer as a module, or stacked structures according to their respective architectures for fine-grained selection. 
Similarly, ${\boldsymbol{\Theta}^l}$ is a positive semi-definite real symmetric matrix and can be eigen-decomposed as $\boldsymbol{\Theta}^l=\mathbf{U}^l \mathbf{\Lambda}^l {\mathbf{U}^l}^\top=\sum_{i=1}^{nk} \lambda_i^l \mathbf{v}_i \mathbf{v}_i^\top$ with $nk$ non-negative eigenvalues $\boldsymbol{\lambda}(\boldsymbol{\Theta}^l) = \{\lambda_1^l,\lambda_2^l, ..., \lambda_{nk}^l\}$. 
Note that a network can be partitioned into modules in flexible ways, for example, by dividing layers within a deep network or components of a network with inherent structures (e.g., attention heads in Transformer or convolutional filters in a CNN).
Since each module has its own mNTK, the integral NTK of a model can be computed as the sum of mNTKs of each module~\citep{yang2021tensor}:
% \begin{equation}
% \label{equ:NTK_mNTK}
%     \begin{aligned}
%     \boldsymbol{\Theta}(\mathcal{X},\mathcal{X})
%     &=\nabla_{\boldsymbol{\theta}} f(\mathcal{X};\boldsymbol{\theta})\nabla_{\boldsymbol{\theta}} f(\mathcal{X};\boldsymbol{\theta})^{\top}
%     =\sum_{p=1}^{m}\nabla_{\boldsymbol{\theta}_p} f(\mathcal{X};\boldsymbol{\theta})\nabla_{\boldsymbol{\theta}_p} f(\mathcal{X};\boldsymbol{\theta})^{\top} \\
%     &=\sum_{l=1}^L\sum_{\boldsymbol{\theta}_p\in \boldsymbol{\theta}^l}\nabla_{\boldsymbol{\theta}_p} f(\mathcal{X};\boldsymbol{\theta})\nabla_{\boldsymbol{\theta}_p}f(\mathcal{X};\boldsymbol{\theta})^{\top}
%     =\sum_{l=1}^L \boldsymbol{\Theta}^l(\mathcal{X},\mathcal{X}).
%     \end{aligned}
% \end{equation}

\begin{equation}
\small
\label{equ:NTK_mNTK}
    \boldsymbol{\Theta}(\mathcal{X},\mathcal{X})
    =J_{\boldsymbol{\theta}}(\mathcal{X})J_{\boldsymbol{\theta}}(\mathcal{X})^\top
    \overset{(i)}{=}\sum_{p=1}^{m}J_{\boldsymbol{\theta_p}}(\mathcal{X})J_{\boldsymbol{\theta_p}}(\mathcal{X})^\top
    \overset{(ii)}{=}\sum_{l=1}^L\sum_{\boldsymbol{\theta}_p\in \boldsymbol{\theta}^l}J_{\boldsymbol{\theta^l}}(\mathcal{X})J_{\boldsymbol{\theta^l}}(\mathcal{X})^\top
    \overset{(iii)}{=}\sum_{l=1}^L \boldsymbol{\Theta}^l(\mathcal{X},\mathcal{X}),
\end{equation}

where $(i)$ decomposes the matrix multiplication into the sum of vector multiplication; $(ii)$ gathers addends by each module; $(iii)$ follows the definition of mNTK.

\subsection{Empirical Analysis}
% This subsection presents detailed empirical studies. 
% We take an over-parameterized and highly-structured model BERT as an example. 
% In order to understand the training dynamics over different modules, we conduct Masked Language Modeling~(MLM) task, which is used for pretraining representations, in different width and depth settings.
In this subsection, we apply BERT to WikiText-2 for language modeling and regard each layer as a module to analyze the properties of eigenvalue distribution of all mNTKs, as well as the modular and temporal variation of eigenvalues during the training process.

% Following the previous works~\citep{huang2020deep, hayou2021stable}, we use normalized NTK to avoid the growing norm in scale-invariant architectures~\citep{li2022robust}, and focus on the consistency of the gradient direction generated by the training data.

% \begin{definition}
% We say that a kernel $\boldsymbol{\Theta}$ is normalized, if $\boldsymbol{\Theta}(x,x)=1$ for all data x. For Neural Tangent Kernel, we normalize it by $\bar{\boldsymbol{\Theta}}(x,x')=\frac{\boldsymbol{\Theta}(x,x')}{\sqrt{\boldsymbol{\Theta}(x,x)\boldsymbol{\Theta}(x',x')}}$.
% \end{definition} 

\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{figure/emp1.png}
    \caption{Training dynamics characterized by layer-wise mNTK of BERT trained on Wikitext-2. (a): The first 16 eigenvalues distribution of layer-wise mNTKs at the $10^{\text{th}}$ epoch. (b): Variation of $\lambda_{\max}$ of layer-wise mNTKs. (c): Variation of $\kappa$ of layer-wise mNTKs during the first $20$ epochs.}
    \label{fig:emp1}
\end{figure}

\noindent\textbf{The principal eigenvalue of mNTK dominates the eigenspectrum of mNTK.}
% As the definition of tangent kernel implies, the spectrum characteristics the learning dynamics of parameters on data features. 
% Figure~\ref{fig:emp1}(a) 
% shows mNTK $\boldsymbol{\Theta}^l$ typically features a single large eigenvalue $\lambda_{\max}^l$ and the gap is large compared with the rest of the spectrum, as~\cite{xiao2020disentangling} found in the integral NTK $\boldsymbol{\Theta}$. So We can quantify the local contribution to optimization by mNTK $\lambda_{\max}$.
% 数量级差异，数目差异（imbalanced）
Figure~\ref{fig:emp1}(a) shows the first 16 eigenvalues of all layer-wise mNTKs at the $10^{\text{th}}$ epoch.
Apparently, the eigenvalue distribution of each layer-wise mNTK is imbalanced where there exists a single large eigenvalue $\lambda_1^l$ ($\lambda_1$ will be denoted by $\lambda_{\max}$ hereafter) and a large number of small eigenvalues. In particular, the largest eigenvalue often has 2 to 4 orders of higher magnitude than that of the rest eigenvalues. 
Based on these findings, we claim that the principal eigenvalue of mNTK dominates the spectrum of the mNTK.  
The phenomenon is also indicated by~\cite{xiao2020disentangling} in terms of NTK. 
Furthermore, according to the connection between NTK and mNTK (Eq.~\ref{equ:NTK_mNTK}), the spectrum of NTK is dominated by the principal eigenvalues of all mNTKs. 
Below, we utilize $\lambda_{\max}$ for fine-grained optimization analysis of over-parameterized model.

% \noindent\textbf{Training is highly asynchronized across modules.}
% As assumed in many infinite-width networks~\citep{seleznova2022neural, Mok_2022_CVPR}, the NTK is deterministic and constant from the initialization. However, this assumption doesn't hold in wide neural networks with complex non-linear structures~\citep{liu2020linearity}, in particular in the early phase of training called rich active regime~\citep{rachwan2022winning}.

% In our experiment, we first look into the variation of layer-wise mNTK. Figure~\ref{fig:emp1}(b) demonstrates that \textcolor{red}{the early layers learn and converge faster in the early stage}, as their $\lambda_{\max}$ is larger and decreases faster, which is consistent with the recently found layer convergence bias~\citep{chenlayer}. 
% Furthermore, $\lambda_{\max}$ of the later layers dominates after the early layers converge. 
% Since later layers tend to capture more task-specific knowledge and early layers encode more general features~\citep{yosinski2014transferable, zhang2019all}, the activeness of later layers depends on the stability of early ones.

% We additionally illustrate the layer-wise condition number $\kappa=\lambda_{\max}/\lambda_{\min}$, which is a widely-used metric of integral NTK~\citep{xu2021knas, xiao2020disentangling}. 
% At the early stage of training, particularly the first 10 epochs, $\kappa$ of the early layers is significantly lower than the later ones. But after that, $\kappa$ of the layers has no significant difference compared with $\lambda_{\max}$, which may not be a sufficient signal for observing the asynchronization between different modules.
% % as many works did~\citep{xu2021knas}.
\noindent\textbf{The variation of principal eigenvalues of mNTKs is highly asynchronous across modules.} 
% 尽管此前工作说ntk是constant，但我们发现max是在变化的
% 不同module的变化趋势不同，浅层先大后小，深层先小后大。在layer的划分下，一个可能的解释是，浅层学xxx
% 另一常用工具是condition number，但是module之间不存在差异，而lambda max持续不同，因此适合细粒度的分析
Figure~\ref{fig:emp1}(b) shows the variation of $\lambda_{\max}$ of all layer-wise mNTKs during the training process. 
It is worth noting that the principal eigenvalues of mNTKs exhibit different trends during the training process. 
Intuitively speaking, NTK (also mNTK) captures the training dynamics throughout the training process, and its principal eigenvector corresponds to the 
% direction of the fastest convergence of loss. 
direction of the steepest descent in loss. 
Specifically, for mNTKs of shallow layers, the magnitude of $\lambda_{\max}$ is large after model initialization, and it decreases and converges fast in the early training stages. A potential explanation is that shallow layers learn common and general features of data samples~\citep{yosinski2014transferable, zhang2019all}, which contribute significantly to model convergence in the early training stages. 
In contrast, for mNTK of the deep layer, the magnitude of $\lambda_{\max}$ is small after initialization 
% ***The figure only appears to show this for one layer.*** 
and gradually increases during training. 
The reason is that deep layers learn unique and data-specific features, relying on the stability of shallow features, which occurs in the later training stages. 

To analyze the training dynamics, condition number is also commonly used~\citep{xu2021knas, xiao2020disentangling}, defined as $\kappa=\lambda_{\max}/\lambda_{\min}$. 
Figure~\ref{fig:emp1}(c) shows the variation of $\kappa$ for different modules during training. 
We observe that the layer-wise condition number exhibits asynchronization among different modules only in the early training stages (especially the first 10 epochs) and $\kappa$ of all modules quickly converges to the same value. 
This reveals that the condition number is hard to provide sustained information for fine-grained optimization analysis, unlike the principal eigenvalue which is capable of capturing the effective information throughout the training process. 


% \noindent\textbf{Temporally dynamic: The variation of the largest eigenvalue of mNTK
% Overfit is accompanied by learning specific or noisy information.} 
% Figure~\ref{fig:emp2} shows the case of overfitting. We conduct the experiments on BERT of 4 transformer encoder layers with 4 heads in each of the layer, trained on the MLM task with only 64 token in each sequence, where the model is prone to overfit. 

% As we can see, though the training perplexity continually decreases, the validation error rebounds at nearly 50 epoch. Simultaneously, the $\lambda_{\max}$ of the modules all converges to a relatively low value. That means the commonality of the parameter updates has been scarce, i.e., the model is likely to learn the features specific to training set or even the noise. ***Is this data set specific? Are small eigenvalue features always unhelpful?***

\noindent\textbf{The temporal variation of the principal eigenvalue of mNTK indicates the generalization ability.} 
In addition to the above analysis depicting the asynchronization between different modules, we examine the temporal variation of the principal eigenvalue given a specific module and establish its connection with the generalization ability. 
In detail, we train the same model using masked modeling on half sequence length, which makes the model prone to overfitting. 
As shown in Figure~\ref{fig:emp2}(a), the validation loss starts to increase from the $45^\text{th}$ epoch while the training loss continually decreases.
Figure~\ref{fig:emp2}(b) presents the temporal variation of the principal eigenvalue for the $3^\text{rd}$, $6^\text{th}$, $9^\text{th}$, and $12^\text{th}$ layers of the model during the training process. 
During the first $45^\text{th}$ epochs, i.e., the non-overfitting stage, the principal eigenvalues of these layers continually decrease. 
However, after the $45^\text{th}$ epoch when the model enters the overfitting stage, the principal eigenvalues converge to a excessively low value. 
This phenomenon suggests that the temporal variation of the principal eigenvalues indicates the generalization ability. 
Additionally, a possible reason for overfitting is that the optimization direction of the model starts to align with the direction of small eigenvalues, which means that the model is learning superfluous features that are too specific or even noise.


% Figure~\ref{fig:emp2} shows the case of overfitting. We conduct the experiments on BERT of 4 transformer encoder layers with 4 heads in each of the layer, trained on the MLM task with only 64 token in each sequence, where the model is prone to overfit. 

% Overfit is accompanied by learning specific or noisy information. 


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figure/emp2.png}
    \caption{Overfitting Case of 4-layer BERT trained by 64 token MLM task.}
    \label{fig:emp2}
\end{figure}

% \begin{wrapfigure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figure/emp2.png}
%     \caption{Overfitting Case of 4-layer BERT trained by 64 token MLM task.}
%     \label{fig:emp2}
% \end{wrapfigure}

\subsection{Theoretical Analysis}
Using the tool of mNTK, we show that the optimization properties of over-parameterized structured models are closely related to the principal eigenvalues of mNTKs.
% trainability and generalization properties ***``Trainability'' and ``generalization'' have not been defined. Different researchers use somewhat different definitions for the sake of experimental convenience.*** 



% \begin{thm}
% \label{thm:mNTK}
% Suppose for any module $\boldsymbol{\theta}^{l}$, $\lambda_{\min}(\boldsymbol{\Theta}^l)=\lambda^l_{nk}>0$. The convergence and generalization of over-parameterized models are respectively related to the spectrum of mNTK as follows:

Suppose for any module $\boldsymbol{\theta}^{l}$, $\lambda_{\min}(\boldsymbol{\Theta}^l)=\lambda^l_{nk}>0$. The convergence and generalization of over-parameterized models are respectively related to the spectrum of mNTK as follows:


(1) Trainability: For a step of gradient descent, to the first order,
% the change to the network’s predictions can be approximated with the first-order Taylor approximation~\citep{jacot2018neural},
loss reduction can be characterized by the directional derivative of the loss function:
\begin{equation}
\label{equ:tra}
\begin{aligned}
\Delta \mathcal{L}
% =\nabla_\mathcal{Z}\mathcal{L}^{\top}\boldsymbol{\Theta}_t\nabla_\mathcal{Z}\mathcal{L}
% =\left(\mathbf{U}_t^{\top} \nabla_{\mathcal{Z}} \mathcal{L}\right)^{\top} \boldsymbol{\Lambda}\left(\mathbf{U}_t^{\top} \nabla_{\mathcal{Z}} \mathcal{L}\right)
% =\sum_{i=1}^{nk} \lambda_{t,i}\left(\mathbf{u}_{t,i}^{\top} \mathcal{Y}\right)^2,
&\overset{(i)}{=}\lim _{\epsilon \rightarrow 0} \frac{\mathcal{L}(\boldsymbol{\theta}+\epsilon \nabla_{\boldsymbol{\theta}} \mathcal{L}(\boldsymbol{\theta}))-\mathcal{L}(\boldsymbol{\theta})}{\epsilon}
\overset{(ii)}{=}\nabla_{\boldsymbol{\theta}} \mathcal{L}(\boldsymbol{\theta})^{\top} \nabla_{\boldsymbol{\theta}} \mathcal{L}(\boldsymbol{\theta}) \\
% &=(\nabla_\mathcal{\boldsymbol{\theta}}\mathcal{Z}\nabla_\mathcal{Z}\mathcal{L}(\boldsymbol{\theta}))^{\top}(\nabla_\mathcal{\boldsymbol{\theta}}\mathcal{Z}\nabla_\mathcal{Z}\mathcal{L}(\boldsymbol{\theta})) \\
% &= \nabla_\mathcal{Z}\mathcal{L}(\boldsymbol{\theta})^{\top}(\nabla_\mathcal{\boldsymbol{\theta}}\mathcal{Z}^{\top}\nabla_\mathcal{\boldsymbol{\theta}}\mathcal{Z})\nabla_\mathcal{Z}\mathcal{L}(\boldsymbol{\theta}) \\
&\overset{(iii)}{=}
\nabla_\mathcal{Z}\mathcal{L}(\boldsymbol{\theta})^{\top}(\nabla_\mathcal{\boldsymbol{\theta}}f(\boldsymbol{\theta})^{\top}\nabla_\mathcal{\boldsymbol{\theta}}f(\boldsymbol{\theta}))\nabla_\mathcal{Z}\mathcal{L}(\boldsymbol{\theta}) \\
% &= \nabla_\mathcal{Z}\mathcal{L}(\boldsymbol{\theta})^{\top}(\boldsymbol{\Theta})\nabla_\mathcal{Z}\mathcal{L}(\boldsymbol{\theta}) \\
&\overset{(iv)}{=}\nabla_\mathcal{Z}\mathcal{L}(\boldsymbol{\theta})^{\top}(\sum_{l=1}^L \boldsymbol{\Theta}^l)\nabla_\mathcal{Z}\mathcal{L}(\boldsymbol{\theta})
% = \sum_{i=1}^{nk} \lambda_{t,i}\left(\mathbf{u}_{t,i}^{\top} \mathcal{Y}\right)^2
% \lesssim \sum_{l=1}^{L} \lambda^l_{1}\left({\mathbf{u}^l_{1}}^{\top} \mathcal{Y}\right)^2,
\overset{(v)}{=} \sum_{l=1}^{L} \sum_{i=1}^{nk} \lambda^l_{i}\left({\mathbf{u}^l_{i}}^{\top} \mathcal{Y}\right)^2,
\end{aligned}
\end{equation}

% (2) Generalization: Fix a failure probability $\delta \in (0,1)$. Then with probability at least $1-\delta$ over the random initialization and the training samples, the network trained by gradient descent has population loss $L_{\mathcal{D}}(f)=\mathbb{E}_{(\mathbf{x}, y) \sim \mathcal{D}}\left[\mathcal{L}\left(f(\mathbf{x}), y\right)\right]$ bounded as:
% \begin{equation}
% \label{equ:gen}
% L_{\mathcal{D}}(f)\leq \sqrt{\frac{2 \mathbf{y}^{\top}(\sum_{l=1}^L \boldsymbol{\Theta}^l)^{-1} \mathbf{y}}{n}}+O\left(\sqrt{\frac{\log \frac{n}{\min_l \delta {\lambda^l_{nk}}}}{n}}\right).
% L_{\mathcal{D}}(f)\leq \sqrt{\frac{2 \mathbf{y}^{\top}(\sum_{l=1}^L \sum_{i=1}^{nk} \lambda_i^l \mathbf{u}_i^l {\mathbf{u}_i^l}^\top)^{-1} \mathbf{y}}{n}}+O\left(\sqrt{\frac{\log \frac{n}{\lambda_{nk} \delta}}{n}}\right).
% L_{\mathcal{D}}(f)\leq \sqrt{\frac{2 \sum_{l=1}^L \sum_{i=1}^{nk}  \frac{1}{\lambda^l_{i}} ({\mathbf{u}^l_{i}}^{\top}\mathcal{Y})^2} {n}}+O\left(\sqrt{\frac{\log \frac{n}{\min_l \delta {\lambda^l_{nk}}}}{n}}\right).
% \end{equation}
% \end{thm}
where $(i)$ follows the definition of derivative; $(ii)$ follows the first order taylor expansion; $(iii)$ follows chain rule of derivation; $(iv)$ follows Eq.~\ref{equ:NTK_mNTK}; $(v)$ follows the eigen-decomposition of mNTK.
% As we can see, the optimization of a structured model is related to every mNTK of modules. Recall the empirical study~\ref{fig:emp1} shows $\boldsymbol{\Theta}^l$ typically features a single large eigenvalue $\lambda_{\max}^l$ and the gap is large compared with the rest of the spectrum. That is, the largest eigenvalue, corresponding to its eigendirection, dominates the update of the module's parameters. So $\lambda_{\max}^l$ can be the nearly equivalent proxy of the spectrum of the module. Under this assumption, we derive Eqs.~\ref{equ:tra}~\ref{equ:gen} into: 
The theorem indicates that the trainability and generalization of a structured model is closely related to the eigenspectrum of mNTKs. 

We first discuss the relation between trainability and principal eigenvalues of mNTKs. 
Based on the first observation of empirical analysis, i.e., the spectrum of each mNTK is dominated by the principal eigenvalues, 
we utilize $\lambda_{\max}$ of mNTKs as the nearly equivalent proxy of the spectrum of mNTKs. Therefore, Eqs.~\ref{equ:tra} is simplified as:
\begin{equation}
\label{equ:tra_m}
\Delta \mathcal{L}
\approx \sum_{l=1}^{L} \lambda^l_{\max}\left({\mathbf{u}^l_1}^{\top} \mathcal{Y}\right)^2.
\end{equation}
% \begin{equation}
% \label{equ:gen_m}
% L_{\mathcal{D}}(f)\leq \sqrt{\frac{2 \sum_{l=1}^L \frac{1}{\lambda^l_{\max}} ({\mathbf{u}^l_{1}}^{\top}\mathcal{Y})^2} {n}}+O\left(\sqrt{\frac{\log \frac{n}{\min_l \delta {\lambda^l_{nk}}}}{n}}\right).
% \end{equation}
% At every step of gradient descent, the model learns the target function faster along the directions corresponding to the larger eigenvalues, driven by those active modules with larger principle eigenvalue of mNTK.
% This conclusion demonstrates the potential for efficient learning, i.e., dispatching limited computational resources to selectively train the modules active with larger $\lambda^l_{\max}$.
The above explanation suggests that the loss decreases faster along the eigenspaces that correspond to larger eigenvalues.
Given the fact that the principal eigenvalues of mNTKs is highly asynchronous across modules, we suggest selectively training the modules that are active with larger $\lambda^l_{\max}$ to achieve efficient learning with limited computational resources. 
% In term of generalization, the larger eigenvalues are the smallest addend of the generalization bound, implying that the features learned by those active modules with with larger $\lambda^l_{\max}$ are easier to generalize. Correspondingly, modules consisting of lower eigenvalues are degraded to learn features specific to training set or noisy information.

% 原先的Generalization Theorem去掉，关于generalization换下面一套故事
% 在上面，根据lmax评估了module的trainability
% lambda的分布 -> 清晰呈现两个峰 小特征值（噪声）居多，大特征值（有效信息）少 且gap巨大 易定义出一个threshold，划分为information/nuisance空间
% 理论上 参数训练时间越长(k越大) -> Redmacher Complexity越大 -> 模型的泛化性越差
% 现有的training scheme下，同时开始同时停止所有参数训练，由于trainability的不同，有些spectrum很低的module (max<threshold, nuisance) 没有学到有用的信息 而凭空增加了Complexity 影响泛化性 
% => 需要Adaptive Training, fix那些nuisance空间的module
% Above we use $\lambda_{\max}$ as the proxy of mNTK to evaluate the trainability of modules. 
% Next, We further build the connection of the asynchronization of modules and generalization issues. 
% Fig~\ref{} plots the histogram of the whole eigenspectrum of all the heads in BERT. The distribution has two distinct intervals. The smaller interval contains significantly more eigenvalues than the larger one, where a huge gap is between them. The distribution can be clearly splited into two parts by a threshold. We term them as information space and nuisance space, as~\cite{oymak2019generalization} did. From the perspective of mNTK, if the principal eigenvalue $\lambda_{\max}$ of a module is less than the threshold, i.e., the whole spectrum falls into the nuisance space, then the module is learning superfluous features , which are trivial to the loss reduction. On the contrary, as long as existing the $\lambda_{\max}$ exceeds the threshold, the module is learning informative features.

\begin{wrapfigure}{R}{0.5\textwidth}
\label{fig:emp3}
\centering
    \includegraphics[width = 0.4\textwidth]{figure/emp3.png}
    \vspace{-10pt}
    \caption{The eigen-spectrum distribution exhibits two distinct regions, termed Infomation space and Nuisance space.}
    \label{fig:importance}
    \vspace{-10pt}
\end{wrapfigure}

% Next, We analyze the impact of modules wit
% principal eigenvalues on the generalization ability, 
% by according to the 

Based on the variation of principal eigenvalues among modules, we further analyze the impact of parameter updates for different modules on the generalization ability of the model. 

The first step is to distinct the modules via principal eigenvalues. 
As shown in Fig~\ref{fig:emp3}, we present the eigen-spectrum distribution of a BERT model at the $10^{\text{th}}$ epoch, by regarding each head as a module while calculating the first 32 eigenvalues for each head. 
Among all 144$\times$32 eigenvalues, the distribution of eigen-spectrum exhibits two distinct regions: 
the left region with a large number of small eigenvalues and the right region with a small number of large eigenvalues (as shown in the first empirical analysis).
According to Equ~\ref{equ:gen_m}, the eigenspaces corresponding to small eigenvalues in the left region only make small contributions to loss descent, while those in the right region make large contributions.
Similar to~\cite{oymak2019generalization}, we refer to the left region as the \textit{nuisance space} and the right region as the \textit{information space}; the two spaces are splited by an eigenvalue threshold. 

% According to the Rademacher complexity-based generalization studies~\citep{arora2019fine}, 
% when the solution of a model has great distance to its  initialization, i.e., the model is trained with much parameter updates, leading to a large Rademacher complexity, as well as a poor generalization ability~\citep{shalev2014understanding}. 
According to theoretical studies on generalization based on Rademacher complexity~\citep{arora2019fine}, 
a model trained with more parameter updates, causing its solution to be located farther from the initialization. 
The model typically has higher Rademacher complexity, which is often associated with a poorer generalization ability~\citep{shalev2014understanding}.



% 
% Under the existing training scheme, where all parameters or modules start and end training together. This leads to the issue that the modules fell into the nuisance space doesn't contribute to the loss reduction but continually being updated, which causes the undesirable rise of Redmacher Complexity, thus impeding the generalization ability. 
Let consider the impact of parameter updates of two modules with variance principal eigenvalues on generalization ability. 
For a module with large eigenvalues, i.e., its principal eigenvalue is greater than the threshold, updating the parameters of this module is advantageous for loss descent. 
Conversely, for module without large eigenvalues, i.e., its principal eigenvalue is smaller than the eigenvalue threshold, it can be considered as fall into the nuisance space with learning superfluous features. 
The parameter updates is useless for loss descent, and even harmful for generalization ability. 
% 
This analysis helps us to answer the aforementioned question: \textit{the existing training scheme overlooks the asynchronization among modules, resulting in inefficient utilization of the computational resource for loss minimization during model training.}

In the following section, we propose an adaptive training scheme that selectively trains modules with larger principal eigenvalues. 
The method saves computational consumption, 
while maintains the generalization capability. 


% find an eigenvalue threshold that can be used to selectively train the modules that are active with larger $\lambda^l_{\max}$. 
% Therefore, we suggest finding a threshold that divides the spectrum into two regions to select which modules should be updated.
% Therefore, 
% 
% The distribution has two distinct intervals. 
% The smaller interval contains significantly more eigenvalues than the larger one, where a huge gap is between them. 
% The distribution can be clearly splited into two parts by a threshold. 
% We term them as information space and nuisance space, as~\cite{oymak2019generalization} did. 
% From the perspective of mNTK, if the principal eigenvalue $\lambda_{\max}$ of a module is less than the threshold, i.e., the whole spectrum falls into the nuisance space, then the module is learning superfluous features, which are trivial to the loss reduction. 
% On the contrary, as long as existing the $\lambda_{\max}$ exceeds the threshold, the module is learning informative features.
% Theoretically, the model trained with more parameter updates tend to have larger distance toward their initial values, which results in larger Rademacher complexity~\citep{arora2019fine}. 
% The large Redmacher complexity makes the model hard to generalize~\citep{shalev2014understanding}.  
% Under the existing training scheme, where all parameters or modules start and end training together. This leads to the issue that the modules fell into the nuisance space doesn't contribute to the loss reduction but continually being updated, which causes the undesirable rise of Redmacher Complexity, thus impeding the generalization ability. 


% Therefore, we propose our method, Modular Adaptive Training, which always updates parts of the modules with better trainability, and stop the training of modules in nuisance space. 
% The proof of the theorem is deferred to Appendix. This indicates that smaller condition number leads to faster model convergence. Suppose $M$ parameters are splited into $L$ modules' weights $w_1, w_2, ..., w_L$, and each of the modules has its own NTK $K_1,K_2,...,K_L$. The integral NTK of the model is the sum up of the modules:
% \begin{equation}
%     \begin{aligned}
%     K(x,x')&=\sum_{p=1}^{M}\nabla_{\theta_p} f(x;\theta)^T\nabla_{\theta_p} f(x';\theta) \\
%     &=\sum_{l=1}^L\sum_{p\in w_l}\nabla_{\theta_p} f(x;\theta)^T\nabla_{\theta_p}f(x';\theta)
%     &=\sum_{l=1}^L K_l(x,x'),
%     \end{aligned}
% \end{equation}
% according to Courant–Fischer theorem~(1905)~\citep{ikebe1987monotonicity}, we have the inequalities:
% \begin{equation}
%     \sum_{l=1}^L{\lambda_1^l}\ge \lambda_1 \ge \lambda_n \ge \sum_{l=1}^L{\lambda_n^l},
% \end{equation}
% from which it follows that $\kappa \le \sum_{l=1}^L{\lambda_1^l} / \sum_{l=1}^L{\lambda_n^l}$.
% If there exists a module $w_s$, whose NTK eigenvalues satisfies ${\lambda^s_1}/{\lambda^s_n} > \sum_{l=1}^L{\lambda_1^l} / \sum_{l=1}^L{\lambda_n^l}$, removing it makes the upper bound on $\kappa$ lower:
% \begin{equation}
% \begin{aligned}
%     \max \kappa' - \max \kappa
%     &= \frac{\sum_{l=1}^L{\lambda_1^l}-\lambda_1^s}{\sum_{l=1}^L{\lambda_n^l}-\lambda_n^s} - \frac{\sum_{l=1}^L{\lambda_1^l}}{\sum_{l=1}^L{\lambda_n^l}}\\
%     &= \frac{(\sum_{l=1}^L{\lambda_1^l}-\lambda_1^s)\sum_{l=1}^L{\lambda_n^l}-(\sum_{l=1}^L{\lambda_n^l}-\lambda_n^s)\sum_{l=1}^L{\lambda_1^l}}{(\sum_{l=1}^L{\lambda_n^l}-\lambda_n^s)\sum_{l=1}^L{\lambda_n^l}} \\
%     &= \frac{\lambda_n^s\sum_{l=1}^L{\lambda_1^l}-\lambda_1^s\sum_{l=1}^L{\lambda_n^l}}{(\sum_{l=1}^L{\lambda_1^l}-\lambda_1^s)\sum_{l=1}^L{\lambda_1^l}} \\
%     &= \frac{\frac{\sum_{l=1}^L{\lambda_1^l}}{\sum_{l=1}^L{\lambda_n^l}} - \frac{\lambda_1^s}{\lambda_n^s}}{\lambda_n^s(\sum_{l=1}^L{\lambda_1^l}-\lambda_1^s)\sum_{l=1}^L{\lambda_1^l}\sum_{l=1}^L{\lambda_n^l}} < 0
% \end{aligned}
% \end{equation}

% This analysis shows that there exists the ill-conditioned module whose condition number may impedes the convergence of the over-parameterized model.

% \textbf{Higher spectrum relates to better generalization.}
% According to the different training dynamics of the eigen-directions, the spectrum can be splited into two spaces like~\citep{oymak2019generalization} does, which helps us derive the properties related to generalization. For a spectrum cutoff $\alpha \in (0, \lambda_1)$, let $r:=r(\alpha)$ denote the index of the smallest eigenvalue above the threshold $\alpha$. We define the information space and nuisance space associated with $K$ as $\mathcal{I}:=span(\{\mathbf{u}_i\}_{i=1}^r)$ and $\mathcal{N}:=span(\{\mathbf{u}_i\}_{i=r+1}^{nk})$. 
% We also define the truncated NTK $\boldsymbol{\Theta}_{\mathcal{I}}=\sum_{i=1}^r \lambda_i \mathbf{u}_i \mathbf{u}_i^\top$. The population loss can be decomposed into two parts by tracking the projection of residual $\boldsymbol{r}_t$ on the two spaces:

% \begin{equation}
% \begin{aligned}
% \mathbb{E} \mathcal{L}(\boldsymbol{\theta})
% =\mathbb{E} \mathcal{L}_{\mathcal{I}}(\boldsymbol{\theta})+\mathbb{E} \mathcal{L}_{\mathcal{N}}(\boldsymbol{\theta})
% =\mathbb{E}\left[\left\|\Pi_{\mathcal{I}}(\boldsymbol{r}_t)\right\|_2^2\right]+
% \mathbb{E}\left[\left\|\Pi_{\mathcal{N}}(\boldsymbol{r}_t)\right\|_2^2\right], 
% \end{aligned}
% \end{equation}

% where $\Pi_{\mathcal{S}}(\boldsymbol{x})$ denotes the projection of a point $\boldsymbol{x}$ onto $\mathcal{S}$. The genralization of randomly initailized networks can be explored by this form of decomposition.

% \begin{thm}
% \label{thm:gen}
% \citep{oymak2019generalization} Let $\zeta, \Gamma, \bar{\alpha}$ be scalars obeying $\zeta\leq 1/2, \Gamma \ge 1, \bar{\alpha} \ge 0$. Consider the training set $\mathcal{X}\times\mathcal{Y}$ where input samples have unit Euclidean norm and the label vector obeys $\|\mathcal{Y}\|_2=\sqrt{n}$ (e.g. one-hot encoding). Consider the activation function $\phi$ obeys $\left|\phi^{\prime}(z)\right|,\left|\phi^{\prime \prime}(z)\right| \leq b$. Assume the truncated NTK $\boldsymbol{\Theta}_{\mathcal{I}}$ is based on a cut-off spectrum value of $\alpha_0=\bar{\alpha} \sqrt[4]{n} \sqrt{k\|\mathcal{X}\|}b$. We run gradient descent in form of~\ref{equ:gd} after $T$ iterations, the generalization error $Err_{\mathcal{D}}(\boldsymbol{\theta}_T)$ is bounded by:
% \begin{equation}
% \begin{aligned}
% Err_{\mathcal{D}}(\boldsymbol{\theta}_T) \leq
% &\underbrace{\frac{2\left\|\Pi_{\mathcal{N}}(\mathcal{Y})\right\|_2}{\sqrt{n}}}_{\text {bias term }}+\underbrace{\frac{12b\sqrt{k}}{\sqrt{n}}\left(\left\|\boldsymbol{\Theta}_{\mathcal{I}}^{-1} \mathcal{Y}\right\|_2+\frac{\Gamma}{\alpha_0}\left\|\Pi_{\mathcal{N}}(\mathcal{Y})\right\|_2\right)}_{\text {variance term }} \\
% &+12\left(1+\frac{\Gamma}{\bar{\alpha} \sqrt[4]{n\|\mathcal{X}\|^2}}\right) \zeta+5 \sqrt{\frac{\log (2 / \delta)}{n}}+2 \mathrm{e}^{-\Gamma},
% \end{aligned}
% \end{equation}
% \end{thm}

% Theorem \ref{thm:gen} tells that the bias and variance term are both mainly influenced by the projection of labels onto the nuisance space, which affects the overall error, while larger range of information space reduces the bound, leading to better generalization. That is, the learned features that fall into the principle parts of the NTK spectrum generalizes better to the testset.

==> old_version/3_method-0513.tex <==
\section{Modular Adaptive Training}
Followed by the theoretical and empirical analysis, we propose our method named Modular Adaptive Training~(MAT), which dynamically trains partial modules of the whole deep network, instead of the existing training scheme. The method consists of two policy: Spatially, the modules are splited into two sets, where the ones with larger contribution to the spectrum are trained in the certain episode; Temporally, we early stop those modules that are susceptible to overfitting.
% Based on the analysis in the previous section, we advocate dynamically optimizing partial modules instead of the overall networks, termed as Modular Adaptive Training~(MAT). 
% MAT consists of spatial policy and temporal policy: Spatially, modules with large contributions to the spectrum of model NTK are optimized while others are freezed; Temporally, modules with small change of eigen-spectrum of module NTK are freezed to avoid overfitting.


\textbf{Spatial Policy.}
Followed by the theoretical analysis, we introduce our methodology to find the modules which contribute to the principle eigenvalues of the integral NTK spectrum. We take nuclear norm as the proxy of NTK spectrum, which equals to the sum of each module's trace:

% We are going to find a component-level binary mask $\bold{m}=\{m^1,m^2,...,m^p\}\in\{0,1\}^p$ which lets $\tilde{\boldsymbol{\Theta}}=\tilde{J}\tilde{J}^T$ where $\tilde{J}=\nabla_{\boldsymbol{\theta}*\bold{m}} f(x;\boldsymbol{\theta})$ and minimizes the variation of $\boldsymbol{\Theta}$, i.e., retrains the principle components of $\boldsymbol{\Theta}$.

\begin{equation}
\|\boldsymbol{\Theta}_t\|_*=Tr(\boldsymbol{\Theta}_t)=\sum_{l=1}^L Tr(\boldsymbol{\Theta}^l_t)
= \sum_{l=1}^L \sum_{i=1}^{nk} \lambda_i (\boldsymbol{\Theta}^l_t)
% \approx \sum_{l=1}^L \lambda_{\max}(\boldsymbol{\Theta}^l_t),
\end{equation}

% Here gives the simple conclusion that those components with larger trace contribute most to the spectrum of the whole NTK.

% $\sum_{l=1}^L \sum_{i=1}^n \lambda_i^l (\boldsymbol{\Theta}^l) \lesssim \sum_{l=1}^L \lambda_{\max}^l (\boldsymbol{\Theta}^l)$.

% \begin{equation}
% \boldsymbol{\Theta}
% =\sum_{l=1}^L \boldsymbol{\Theta}^l
% =\sum_{l=1}^L \sum_{i=1}^n \lambda_i^l \mathbf{u}^l_i {\mathbf{u}_i^l}^{\top}
% \lesssim \sum_{l=1}^L \lambda_{\max}^l \mathbf{u}^l_1 {\mathbf{u}_1^l}^{\top}.
% \end{equation}
Given the eigenvalues of module-level NTK over all modules $\boldsymbol{\tilde{\Lambda}}=\{\lambda_i^l\}_{i,l=1}^{nk,L}$, let $\tilde{\lambda}_{\max}, \tilde{\lambda}_{\min}$ denote the maximum and minimum value of the set $\boldsymbol{\tilde{\Lambda}}$.
Motivated by~\cite{oymak2019generalization}, we propose a cutoff $\alpha$ obeying $0\leq \alpha \leq \tilde{\lambda}_{\max}$,
% let $r:=r(\alpha)$ denote the index of the smallest eigenvalue above the threshold $\alpha$.
then define the information and nuisance module sets associated with 
\begin{equation}
\mathcal{I}_t=\{\boldsymbol{\theta}^l|\lambda_{\max}(\boldsymbol{\Theta}^l_t)\geq \alpha\}, \mathcal{N}_t=\{\boldsymbol{\theta}^l|\lambda_{\max}(\boldsymbol{\Theta}^l_t) < \alpha\}.   
\end{equation}
Therefore, at each training episode, modules are split into two parts. Only the gradients of modules in $\mathcal{I}_t$ are computed. In our empirical study, $\alpha$ can be assigned by a ratio over the normalized spectrum distribution:
\begin{equation}
\label{equ:spatial}
\alpha=\tilde{\lambda}_{\min}+(\tilde{\lambda}_{\max}-\tilde{\lambda}_{\min})\times \tau,
\end{equation}
where $\tau \in (0,1)$ is relatively stable for splitting two clusters over the training process for a certain model and dataset. Therefore, $\tau$ can be empirically set at the early stage of training after warming up, or further trained by a meta network. 

\textbf{Temporal Policy.} As the empirical study shows, the overfit is accompanied with the $\lambda_{\max}$ of those modules converging to excessively low value. Based on this observation, We heuristically design the policy on temporal level. For each module, we record the largest eigenvalue of NTK after warming up as the initial value $\lambda_{\max}(\boldsymbol{\Theta}_0^l)$. At following training episode $t$, we compute the variation $\Delta^l_t=|\lambda_{\max}(\boldsymbol{\Theta}_t^l)-\lambda_{\max}(\boldsymbol{\Theta}_0^l)|$. The module is early stopped into $\mathcal{N}$ set if the difference of the variation at two subsequent episode relative to the initial variation is smaller than a defined threshold:
\begin{equation}
\label{equ:temporal}
\frac{|\Delta^l_t-\Delta^l_{t-1}|}{\Delta^l_1}<\epsilon.
\end{equation}
% Specifically, we early stop the training of the components whose decrease of $\lambda_{\max}$ is lower than a threshold $\epsilon$. 

% \textbf{Approximation.} \textcolor{red}{**TODO**}
% Alternatively, we can approximate the nuclear norm of NTK even without back-propagation by random sampling, which allows more data samples to calculate. The trace of NTK equals to the squared Frobenius norm of Jacobian with respect to time $t$ in form of finite difference method:

% \begin{equation}
% \|\boldsymbol{\Theta}_t\|_*=Tr(\boldsymbol{\Theta}_t)=\|\nabla_{\boldsymbol{\theta}_t}f(\mathcal{X}; \boldsymbol{\theta}_t)\|^2_F
% \end{equation}

% \begin{equation}
% \begin{aligned}
% \mathbb{E}_{\Delta \boldsymbol{\theta} \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{I})}\left[\left\|f\left(\mathcal{X} ; \boldsymbol{\theta}_t\right)-f\left(\mathcal{X} ; \boldsymbol{\theta}_t+\Delta \boldsymbol{\theta}\right)\right\|_2^2\right]
% % & \approx \mathbb{E}_{\Delta \boldsymbol{\theta}}\left[\left\|\nabla_{\boldsymbol{\theta}_0} f\left(\mathcal{X} ; \boldsymbol{\theta}_0\right) \Delta \boldsymbol{\theta}\right\|_2^2\right] \\
% % &= \sum_{i, j}\left[\nabla_{\boldsymbol{\theta}_0} f\left(\mathcal{X} ; \boldsymbol{\theta}_0\right)\right]_{i, j}^2 \mathbb{E}\left[\Delta \theta_j \Delta \theta_j\right] \\
% &\approx \left\|\nabla_{\boldsymbol{\theta}_t} f\left(\mathcal{X} ; \boldsymbol{\theta}_t\right)\right\|_F^2 .
% \end{aligned}
% \end{equation}

\begin{algorithm}
\label{alg:over}
\caption{Modular Adaptive Training}
\begin{algorithmic}
    \REQUIRE
    training data $\{\mathbf{x}_i, \mathbf{y}_i\}_{i=1}^n$, sample number $k$, modules set $\mathcal{C}$, spatial threshold $\tau$, temporal threshold $\epsilon$.

    % \STATE
    % $\mathcal{A}_0=\mathcal{C}$
    % \STATE
    % $\mathcal{N}_0=\varnothing$

    \WHILE{not converged and $|\mathcal{I}_t|>0$}
    \STATE
    Compute $\nabla_{\boldsymbol{\theta}} f(\mathbf{x};\boldsymbol{\theta})$ for samples $\{\mathbf{x}_i, \mathbf{y}_i\}_{i=1}^k$
    \hfill
    $\triangleright$
    \textit{ Approximated Jacobian for NTK}
    \STATE
    $\tilde{\boldsymbol{\Lambda}}=\varnothing$
    \FOR{$\boldsymbol{\theta}^l$ in $\mathcal{C}$}
        \STATE
        $\boldsymbol{\Theta}^l=\nabla_{\boldsymbol{\theta}^l} f(\mathbf{x};\boldsymbol{\theta})\nabla_{\boldsymbol{\theta}^l}f(\mathbf{x};\boldsymbol{\theta})^{\top}$
        \hfill
        $\triangleright$
        \textit{ Modular NTK}
        \STATE
        Compute eigen-decomposition $\boldsymbol{\Theta}^l=\mathbf{U}^l \boldsymbol{\Lambda}^l {\mathbf{U}^l}^\top$
        \STATE
        $\Delta^l_t=|\lambda_{\max}(\boldsymbol{\Theta}^l)-\lambda_{\max}(\boldsymbol{\Theta}_0^l)|$
        \STATE
        $\tilde{\boldsymbol{\Lambda}}=\tilde{\boldsymbol{\Lambda}} \cup \mathbf{\Lambda}^l$
    \ENDFOR

    % \STATE
    % $\tilde{\lambda}_{\max},\tilde{\lambda}_{\min} =\max(\tilde{\boldsymbol{\Lambda}}),\min(\tilde{\boldsymbol{\Lambda}})$

    \STATE
    $\alpha=\min(\tilde{\boldsymbol{\Lambda}})+(\max(\tilde{\boldsymbol{\Lambda}})-\min(\tilde{\boldsymbol{\Lambda}}))\times \tau$
    
    \STATE
    $\mathcal{N}=\{\boldsymbol{\theta}^l|\lambda_{\max}(\boldsymbol{\Theta}^l_t) < \alpha\}$
    \hfill
    $\triangleright$
    \textit{ Spatial policy Eq.~\ref{equ:spatial}}

    \STATE
    $\mathcal{N}=\mathcal{N} \cup \{\boldsymbol{\theta}^l|\frac{|\Delta^l_t-\Delta^l_{t-1}|}{\Delta^l_1}<\epsilon\}$
    \hfill
    $\triangleright$
    \textit{ Temporal policy Eq.~\ref{equ:temporal}}
    
    \STATE
    $\mathcal{I}=\mathcal{C}-\mathcal{N}$
    \FOR{each batch $\mathbf{x}, \mathbf{y}$ in $\{\mathbf{x}_i, \mathbf{y}_i\}_{i=1}^n$}
        \FOR{$\boldsymbol{\theta}^l$ in $\mathcal{I}$}
            \STATE
            $\boldsymbol{\theta}^l=\boldsymbol{\theta}^l-\eta\nabla_{\boldsymbol{\theta}^l}\mathcal{L}(f(\mathbf{x};\boldsymbol{\theta}),\mathbf{y})$
        \ENDFOR
    \ENDFOR
    \ENDWHILE
\end{algorithmic}
\end{algorithm}

The overall algorithm is summarized in Algorithm~\ref{alg:over}.
